Multi-level Explanation of Deep Reinforcement Learning-based Scheduling

Dependency-aware job scheduling in the cluster is NP-hard. Recent work shows that Deep Reinforcement Learning (DRL) is capable of solving it. It is difficult for the administrator to understand the DRL-based policy even though it achieves remarkable performance gain. Therefore the complex model-based scheduler is not easy to gain trust in the system where simplicity is favored. In this paper, we give the multi-level explanation framework to interpret the policy of DRL-based scheduling. We dissect its decision-making process to job level and task level and approximate each level with interpretable models and rules, which align with operational practices. We show that the framework gives the system administrator insights into the state-of-the-art scheduler and reveals the robustness issue in regards to its behavior pattern.

==> Sections/Section_3_prelimaries.tex <==
% 1. DRL-based Scheduler: definition of scheduling problem, the Decima scheduler, the challenge of applying without understanding the policy.
% 2. the tree-based explanation framework, how to choose the features for node split. While it's hard to split, then incorporate the compositional model (RM) for decision making, job selecting, and rule-based node selection.
\textbf{DRL-based scheduler.} A set of jobs $\mathcal{J}$ are submitted by users on a set of computation nodes $\mathcal{E}$. Each job $J \in \mathcal{J}$ (represented as DAG)  contains a set of task nodes $\mathcal{N}$. There are multiple homogeneous tasks in each task node, running the same code on a different dataset. At time stage $t$, the DRL observes job \emph{state} $S_t$, which is composed of raw features in the DAG, e.g. task numbers and estimated per-task run time in each task node, and summary information generated after aggregation by GNNs. \emph{Policy} $f$ is encoded by DNN and maps the state to the \emph{action} $A_t$ as $f: S_t \rightarrow A_t$.  Generally, 
$f$ gives a score for each task node of all jobs, and the action assigns the task from the node with the largest score for execution. Since tasks in a node are homogeneous, the scheduler does not differentiate between them. So the size of action space is $\sum{|\mathcal{N}|}$. The whole process is shown in Figure~\ref{fig:explanation_framework}.     

\textbf{Multi-level explanation framework.} In order to explain the DRL policy $f$, an approximate model $g$ should derive actions as $g: S_t \rightarrow A^*_t$, and guarantee high similarity between $A_t$ and $A^*_t$, at all scheduling time stages $t$. However, direct use of interpretable models, e.g. sparse linear model \cite{Ustun16supersparse}, rules \cite{benjamin15interpretable} or  trees \cite{breiman1984classification}, can hardly approach the DRL agent action. 
So we decompose job schedule to two distinctive processes as first selecting a candidate job from the queue with $g_j$ (inter-job decision), and then selecting a task node in the job and executing its task with $g_n$ (intra-job decision), as shown by dash arrows in Figure ~\ref{fig:explanation_framework}. At schedule time stage $t$, $g_j$ maps state $S_t$ to a specific job $J_t$ as $g_j: S_t \rightarrow J_t$, while $g_n$ maps the chosen job $J_t$ to a task node $N_t$ as $g_n: J_t \rightarrow N_t$. The output space size of $g_j$ is $|\mathcal{J}|$, and of $g_n$ is $|\mathcal{N}|$. As $|\mathcal{J}| + |\mathcal{N}| \ll \sum |\mathcal{N}|$, the space size is decreased in magnitude.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/framework_nips.pdf}
    \caption{The DRL-based job scheduler and the multi-level explanation framework.}
    \label{fig:explanation_framework}
\end{figure}




